Data Collection-free Masked Video Modeling

Pre-training video transformers generally requires a large amount of data, presenting significant challenges in terms of data collection costs and concerns related to privacy, licensing, and inherent biases. Synthesizing data is one of the promising ways to solve these issues, yet pre-training solely on synthetic data has its own challenges. In this paper, we introduce an effective self-supervised learning framework for videos that leverages readily available and less costly static images. Specifically, we define the Pseudo Motion Generator (PMG) module that recursively applies image transformations to generate pseudo-motion videos from images. These pseudo-motion videos are then leveraged in masked video modeling. Our approach is applicable to synthetic images as well, thus entirely freeing video pre-training from data collection costs and other concerns in real data. Through experiments in action recognition tasks, we demonstrate that this framework allows effective learning of spatio-temporal features through pseudo-motion videos, significantly improving over existing methods which also use static images and partially outperforming those using both real and synthetic videos. These results uncover fragments of what video transformers learn through masked video modeling.

==> figures/top.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{assets/proposed_pvg.pdf}

    \caption{
        \begin{small}
        Placeholder for Figure 1.
        \end{small}
    }

    \vspace{-5mm}
    \label{fig:proposed_pvg}
\end{figure}

==> section/6_conclusion.tex <==
\vspace{-1mm}
\section{Conclusion}

In this paper, we introduced a self-supervised framework
for pre-training video transformers solely with synthetic images.
Our framework eliminates the costs associated with collecting video data
and addresses concerns related to privacy, licensing, and biases inherent in real data.
Our experiments have demonstrated that our method
not only outperforms existing pre-training methods with static images
but also partially outperforms existing works with synthetic videos.
These results unveiled segments of what masked autoencoders learn from videos.


==> tables/compare_pseudo_video_generation_method_fdssl.tex <==
\begin{table*}[t]

\caption{
    \begin{small}
    人工画像を用いた事前学習において,擬似動画の生成方法ごとの,行動認識タスクの性能比較.
    学習に使う動画数は全て10,000枚で統一している.
    \end{small}
}
\label{tab:result}
\centering
\small
\begin{tabular}{ccccc}
\multirow{2}{*}{Method} & Pretraining       & \multicolumn{3}{c}{Supervsied Finetuning} \\
                        & Dataset           & UCF-101     & HMDB-51 & Diving48 \\ \hline
Static Video   & \multirow{3}{*}{FractalDB} & 44.6        & 22.4    &          \\
Ours           &                            & 72.3        & 36.1    &          \\
Ours w/ mixup  &                            & 73.3        & 34.6    &          \\ \hline
Static Video   & \multirow{3}{*}{Shaders1k} & 71.5        & 35.4    &          \\
Ours           &                            & 85.8        & 54.0    &          \\
Ours w/ mixup  &                            & 88.5        & 60.3    &          \\ \hline
Static Video   & \multirow{3}{*}{Visual Atom}& 62.3       & 26.5    &          \\
Ours           &                            & 80.0        & 46.0    &          \\
Ours w/ mixup  &                            & 83.4        & 51.3    &          \\ \hline

\end{tabular}
\end{table*}


==> tables/comparison_of_natural_datasets.tex <==
\begin{table}[t]
\caption{
    \begin{small}
    Pretraining on UCF-101, HMDB-51 and ImageNet.
    \end{small}
}
\label{tab:result}

\centering
\small
\begin{tabular}{cccc}
\multicolumn{2}{c}{Pretraining} & \multicolumn{2}{c}{Supervised Finetuning} \\
Dataset       & \#data          & UCF101 & HMDB51 \\ \hline
no extra data & -               & 88.0   & 55.8  \\
ImageNet      & 10,000          & 88.3   & 59.1  \\
ImageNet      & 100,000         & 88.9   & 61.0  \\ \hline

\end{tabular}
\end{table}

==> tables/pvg_as_video_augmentation.tex <==
\begin{table}[t]
\caption{
    \begin{small}
    todo
    % 提案する擬似動画生成手法を、事前学習におけるデータ拡張として使用した際の性能比較。
    \end{small}
}
\label{tab:result}

\centering
\small
\begin{tabular}{cc}
Pretraining Data         & HMDB-51 \\ \hline
Raw Video                & 62.6    \\
Pseudo Video             & 55.9    \\
Raw Video + Pseudo Video & \textbf{64.2} \\ \hline

\end{tabular}
\end{table}

==> tables/what_videomae_learns.tex <==
\begin{table}[t]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{.49\textwidth}
\scriptsize
\centering
\caption{VideoMAE pre-training for 2000 epochs when using the subset of HMDB51 and UCF101}
\begin{tabular}{ccc}
\toprule[1.2pt]
Video                                & HMDB51   & UCF101 \\
\midrule[0.5pt]
Top 50\% of frame difference         & 32.9          & 68.7   \\
Bottom 50\% of frame difference      & 32.2          & 69.3   \\
25\% $\sim$ 75\% of frame difference & \textbf{33.5} & \textbf{71.0}   \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:what_video_learns1}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.01\textwidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{minipage}{.49\textwidth}

% \scriptsize
% \centering
% \caption{VideoMAE pre-training for 2000 epochs when using 10k videos from K400.}
% % 分布がたまたま重なった可能性。
% \begin{tabular}{ccc}
% \toprule[1.2pt]
% A subset of K400                    & HMDB51  & UCF101 \\
% \midrule[0.5pt]
% high frame difference   & 38.7      & 71.7   \\
% low frame difference    & 40.9      & 75.0   \\
% medium frame difference & 40.0      & 72.2   \\
% \bottomrule[1.2pt]
% \end{tabular}
% \label{tab:what_video_learns2}

% \end{minipage}

\end{table}
